Density Matrices for Metaphor Understanding

In physics, density matrices are used to represent mixed states, i.e. probabilistic mixtures of pure states. This concept has previously been used to model lexical ambiguity. In this paper, we consider metaphor as a type of lexical ambiguity, and examine whether metaphorical meaning can be effectively modelled using mixtures of word senses. We find that modelling metaphor is significantly more difficult than other kinds of lexical ambiguity, but that our best-performing density matrix method outperforms simple baselines as well as some neural language models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{197}
\providecommand{\publicationstatus}{A. D\'iaz-Caro and V. Zamdzhiev (Eds.):\\
Quantum Physics and Logic 2024 (QPL 2024)\\
EPTCS 406, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.406.9}{10.4204/EPTCS.406.9}}
\pdfoutput=1

